Improved Order Analysis and Design of Exponential Integrator for Diffusion Models Sampling

Efficient differential equation solvers have significantly reduced the sampling time of diffusion models (DMs) while retaining high sampling quality. Among these solvers, exponential integrators (EI) have gained prominence by demonstrating state-of-the-art performance. However, existing high-order EI-based sampling algorithms rely on degenerate EI solvers, resulting in inferior error bounds and reduced accuracy in contrast to the theoretically anticipated results under optimal settings. This situation makes the sampling quality extremely vulnerable to seemingly innocuous design choices such as timestep schedules. For example, an inefficient timestep scheduler might necessitate twice the number of steps to achieve a quality comparable to that obtained through carefully optimized timesteps. To address this issue, we reevaluate the design of high-order differential solvers for DMs. Through a thorough order analysis, we reveal that the degeneration of existing high-order EI solvers can be attributed to the absence of essential order conditions. By reformulating the differential equations in DMs and capitalizing on the theory of exponential integrators, we propose refined EI solvers that fulfill all the order conditions, which we designate as Refined Exponential Solver (RES). Utilizing these improved solvers, RES exhibits more favorable error bounds theoretically and achieves superior sampling efficiency and stability in practical applications. For instance, a simple switch from the single-step DPM-Solver++ to our order-satisfied RES solver when Number of Function Evaluations (NFE) $=9$, results in a reduction of numerical defects by $25.2\%$ and FID improvement of $25.4\%$ (16.77 vs 12.51) on a pre-trained ImageNet diffusion model.

==> figure/algo/single_second_full.tex <==
\begin{algorithm}[t]
    \footnotesize
    \captionof{algorithm}[single-step]{\atphantom\ \ DEIS++ Single Step Second order}
    \begin{spacing}{1.1}
    \begin{algorithmic}[1]
      \AProcedure{SingleSecondSampler}{$D_\theta, ~t_{i \in \{0, \dots, N\}}, c_{2}$}
        % \AState{\bf calcualte} $a_{21},b_1,b_2$ with~\cref{eq:deispp-single-2} and $c_2$
        \AState{{\bf sample} $\vx_0 \sim \mathcal{N} \big( \mathbf{0}, ~t^2_0 \mathbf{I} \big)$}
            \AComment{Generate initial sample at $t_0$}
        \AFor{$i \in \{0, \dots, N-1\}$}
        %     \AComment{Solve Eq.~\ref{eq:odescale} over $N$ time steps}
            \AState{$\lambda_{i+1}, \lambda_i \gets \log(t_{i+1}),  \log( t_i)$}
            \AState{$h_i \gets \lambda_{i+1} - \lambda_i$}
                \AComment{Step length}
            \AState{$a_{21}, b_1, b_2 \gets$ \cref{eq:deispp-single-2} with $c_2$}
                \AComment{Runge Kutta coeffients}
          \AState{$\vd_i \gets D_\theta(\vx_i; t_i) -\vx_i $}
                \AComment{Evaluate $\diff\vx / \diff \lambda$ at $(\vx,\,\lambda_i)$}
          \AState{$(\vx'_i,\,t'_i) \gets (\vx_i + a_{21} h \vd_i,\,\exp(\lambda_i + c_2 h))$}
                \AComment{Additional evaluation point}
          \AState{$\vd'_i \gets D_\theta(\vx'_i; t'_i) -\vx'_i $}
                \AComment{Evaluate $\diff\vx / \diff \lambda$ at $(\vx'_i,\,\lambda'_i)$}
          \AState{$\vx_{i+1} \gets \vx_i + h(b_1 \vd + b_2 \vd')$}
        \EndFor
        \AState{\textbf{return} $\vx_N$}
            \AComment{Return noise-free sample at $t_N$}
      \EndProcedure
    \end{algorithmic}
    \end{spacing}
    \label{alg:deispp-single-second}
    \end{algorithm}
    

==> figure/algo/single_third.tex <==
\begin{algorithm}[t]
    \footnotesize
    \captionof{algorithm}[single-step]{\atphantom\ \our Third order Single Update Step with $c_2,c_3$}
    \begin{spacing}{1.1}
    \begin{algorithmic}[1]
        \AProcedure{SingleUpdateStep}{$\vx_i, t_i, t_{i+1}$}
            \AState{$\lambda_{i+1}, \lambda_i \gets \log(t_{i+1}),  \log( t_i)$}
            \AState{$h_i \gets \lambda_{i+1} - \lambda_i$}
                \AComment{Step length}
            \AState{$a_{21}, a_{31}, a_{32}, b_1, b_2,b_3 \gets$ \cref{eq:deispp-single-3} with $c_2,c_3$}
                \AComment{Runge Kutta coeffients}
          \AState{$\vd_i \gets D_\theta(\vx_i; t_i) -\vx_i $}
                \AComment{Evaluate $\diff\vx / \diff \lambda$ at $(\vx,\,\lambda_i)$}
          \AState{$(\vx'_i,\,t'_i) \gets (\vx_i + a_{21} h \vd_i,\,\exp(\lambda_i + c_2 h))$}
                \AComment{Additional evaluation point}
          \AState{$\vd'_i \gets D_\theta(\vx'_i; t'_i) -\vx'_i $}
                \AComment{Evaluate $\diff\vx / \diff \lambda$ at $(\vx'_i,\,\lambda'_i)$}
          \AState{$(\vx''_i,\,t''_i) \gets (\vx_i + a_{31}h \vd_i + a_{32}h\vd_i',\,\exp(\lambda_i + c_3 h))$}
                \AComment{Additional evaluation point}
          \AState{$\vd''_i \gets D_\theta(\vx''_i; t''_i) -\vx''_i $}
                \AComment{Evaluate $\diff\vx / \diff \lambda$ at $(\vx''_i,\,\lambda''_i)$}
            \AState{$\vx_{i+1} \gets \vx_i + h(b_1 \vd + b_2 \vd' + b_3 \vd'' )$}
        \AState{\textbf{return} $\vx_{i+1}$}
      \EndProcedure
    \end{algorithmic}
    \end{spacing}
    \label{alg:eis-single-third}
\end{algorithm}

==> figure/algo/single_third_full.tex <==
\begin{algorithm}[t]
    \footnotesize
    \captionof{algorithm}[single-step]{\atphantom\ \ DEIS++ Single Step Third order}
    \begin{spacing}{1.1}
    \begin{algorithmic}[1]
      \AProcedure{SingleThirdSampler}{$D_\theta, ~t_{i \in \{0, \dots, N\}}, c_{2}, c_{3}$}
        \AState{{\bf sample} $\vx_0 \sim \mathcal{N} \big( \mathbf{0}, ~t^2_0 \mathbf{I} \big)$}
            \AComment{Generate initial sample at $t_0$}
        \AFor{$i \in \{0, \dots, N-1\}$}
        %     \AComment{Solve Eq.~\ref{eq:odescale} over $N$ time steps}
            \AState{$\lambda_{i+1}, \lambda_i \gets \log(t_{i+1}),  \log( t_i)$}
            \AState{$h_i \gets \lambda_{i+1} - \lambda_i$}
                \AComment{Step length}
            \AState{$a_{21}, a_{31}, a_{32}, b_1, b_2,b_3 \gets$ \cref{eq:deispp-single-3} with $c_2,c_3$}
                \AComment{Runge Kutta coeffients}
          \AState{$\vd_i \gets D_\theta(\vx_i; t_i) -\vx_i $}
                \AComment{Evaluate $\diff\vx / \diff \lambda$ at $(\vx,\,\lambda_i)$}
          \AState{$(\vx'_i,\,t'_i) \gets (\vx_i + a_{21} h \vd_i,\,\exp(\lambda_i + c_2 h))$}
                \AComment{Additional evaluation point}
          \AState{$\vd'_i \gets D_\theta(\vx'_i; t'_i) -\vx'_i $}
                \AComment{Evaluate $\diff\vx / \diff \lambda$ at $(\vx'_i,\,\lambda'_i)$}
          \AState{$(\vx''_i,\,t''_i) \gets (\vx_i + a_{31}h \vd_i + a_{32}h\vd_i',\,\exp(\lambda_i + c_3 h))$}
                \AComment{Additional evaluation point}
          \AState{$\vd''_i \gets D_\theta(\vx''_i; t''_i) -\vx''_i $}
                \AComment{Evaluate $\diff\vx / \diff \lambda$ at $(\vx''_i,\,\lambda''_i)$}
            \AState{$\vx_{i+1} \gets \vx_i + h(b_1 \vd + b_2 \vd' + b_3 \vd'' )$}
        \EndFor
        \AState{\textbf{return} $\vx_N$}
            \AComment{Return noise-free sample at $t_N$}
      \EndProcedure
    \end{algorithmic}
    \end{spacing}
    \label{alg:deispp-third-second}
\end{algorithm}

==> figure/viz/dfif.tex <==
\begin{figure}[!htp]
    \centering
    \includegraphics[width=4cm]{example-image-a}
    \includegraphics[width=4cm]{example-image-a}
    \caption{(1) FID wit NFE. (2) Fixed NFE, trade-off between FID and CLIP score.}
    \label{fig:dfif}
\end{figure}

==> figure/viz/poly_fit.tex <==
\begin{figure}[!htp]
    \centering
    \includegraphics[width=4cm]{figure/tikz_pdf/poly_ab.pdf}
    \includegraphics[width=4cm]{figure/tikz_pdf/poly_am.pdf}
    \caption{Fitting polynomial with Adam Adams-Bashforth for predictor and with Adams-Moulton for corrector.}
    \label{fig:poly_fit}
\end{figure}

==> figure/viz/stochastic_sampler.tex <==
\begin{figure}[!htp]
    \centering
    \includegraphics[width=4cm]{figure/tikz_pdf/stochastic_graph.pdf}
    \caption{Illustration of a stochastic sampler~\qsh{label error, remove me if run out of space}.}
    \label{fig:stochastic_sampler}
\end{figure}

==> sections/body_2.tex <==
\section{
    Extention to noise prediction model
}

Though ODE based on noise prediction model~\cref{eq:eps-ode} has a different formulation compared with~\cref{eq:semi_ode}, we can apply similar order 
 analysis for~\cref{eq:eps-ode}. 
We start our analysis from the exact ODE solution.
The variation-of-constant formula gives the solution
\begin{equation}~\label{eq:sol-eps-ode}
    \vx(\sigma_{n+1}) = \vx(\sigma_n) + \int_{\sigma_n}^{\sigma_{n+1}} \eps_\theta(\vx(\sigma), \sigma) \diff \sigma.
\end{equation}
Similarly, with the change of variable $\lambda = \log \sigma$, we can reformulate~\cref{eq:sol-eps-ode} 
\begin{align}\label{eq:eps-lambda}
    \vx(\lambda + h) 
    % &= \vx(\lambda) + \int_{\lambda}^{\lambda + h} \eps_\theta(\vx(e^\tau), e^\tau) e^{\tau} \diff \tau  
    = \vx(\lambda) + e^{\lambda + h} \int_{0}^{h} e^{\tau - h} \eps_\theta(\vx(e^{\lambda + \tau}), e^{\lambda + \tau}) \diff \tau.
\end{align}
Upon comparing with~\cref{eq:voc}, we observe an interesting parallelism: the intractable integration found in~\cref{eq:eps-lambda} bears a striking resemblance to the structure in~\cref{eq:voc}.
\qsh{GPT4 is so decent. Upon juxtaposition with~\cref{eq:voc}, it becomes discernible that the intractable integration delineated in~\cref{eq:eps-lambda} mirrors the precise structural form inherent in~\cref{eq:voc}. }
This similarity is marked by a metamorphosis of the nonlinearity function from a data prediction model $\mD_\theta(\vx, \sigma)$ to a noise prediction model $\eps_\theta(\vx, \sigma)$. 
Therefore, we can apply a similar error analysis developed in~\cref{sub:ode-error-analysis} for approximating intractable integration present in~\cref{eq:eps-lambda}. 
We summarize the main results in the following theorem,

\begin{thm}
    Solving  ODE~\cref 
    with the numerical scheme follows
    \begin{equation}
        \vx_{n+1} = \vx_n + e^{\lambda_n + h}h_n \sum_{i=1}^s b_i(-h_n) \ve_{ni} \quad 
        \vx_{ni}  = e^{-c_i h_n} \vx_n + e^{\lambda_n + c_ih} h_n \sum_{j=1}^{i-1} a_{ij}(-h_n) \ve_{nj}
    \end{equation}
    with $\ve_{nj} = \epsilon_\theta(\vx_{nj}, e^{\lambda_n + c_j h_n})$.
\end{thm}


$
\vy(\lambda)  = \frac{\vx(\lambda)}{\sigma({\lambda})}
$

$
\diff \vy = -\vy + \eps_\theta(\vy, \lambda) \diff \lambda
$

% with a non-zero weight $e^{\lambda + h}$.


==> sections/body_bank.tex <==
% As showon in~\cref{}, nonlinear function 

Compared with $\epsilon_\theta(\vx, \sigma)$ in ~\cref{eq:eps-ode}, the nonlinearity origins from the denoiser $D_\theta(\vx, \sigma)$. Similarly, we visualize the ODE function $D_\theta(\vx, \sigma)$ along the solution trajectory $\vx(t)$ in \cref{fig:ode-function}.
Compared with $\epsilon_\theta(\vx(t), \sigma(t))$, we observe that the ODE function $D_\theta(\vx(t), \sigma(t))$ is less veratile and the derivative of ODE function $D_\theta(\vx(t), \sigma(t))$ is better behavied.



The main challenges of solving diffusion flow ODE is origin from nonlinear denoiser, which evolves along solution trajectory $\vx(\sigma)$.
Though~\cref{eq:simple-ode,eq:eps-ode} is shown to have substantial curvature and its solution trajectory $\vx(\sigma)$ is close to a linear, it turns out function evaluation along trajectories is very high nonlinear and cause stiffness for either $\vf_\mD(\sigma) := \mD_\theta(\vx(\sigma), \sigma)$ or $\vf_\epsilon(\sigma) := \eps_\theta(\vx(\sigma), \sigma)$. 



However, such requirments have not been verified in diffusion models settings, despite the existence of high-nolinearity of network and uncontrollable denoiser training.

Both EDM~\citep{karras2022elucidating} and RK-DEIS~\citep{eq:eps-ode} treat the integrant in ODEs as a blackbox function and rely on existing Runge Kutta method to solve ODEs. Thus, the order conditions are trivially satisfied.

Empirically, \citet{lu2022dpmp} show solvers developed with data prediction model $\mD_\theta$ show better stability and sampling quality over noise prediction model $\epsilon_\theta$, expecially for guided diffusion models.

Another deisgn axis lies in splitting ODE integrant into a known linear term and another nonlinear term.
To solve the semi-linear ODE, \citet{zhang2022fast,lu2022dpmp} leverage ideas from exponential integrators and propose tailored algorithm for diffusion model and achieves state-of-the-art sampling performance.

% Specially, 
% With analytical treatment for the linear term, 
% and treat the linear term ly.



% The propsed DPM-Solver$++$ further incorpolates ideas from exponential integrators to accelerate diffusion model sampling.




% To see the point, we visualize the ODE function $\epsilon_\theta(\vx, \sigma)$ along the solution trajectory $\vx(t)$ in \cref{fig:ode-function}.
% With SOTA trained diffusion model~\cite{}, we observe that the trajectory $\epsilon_\theta(\vx(t), \sigma(t))$ is highly nonlinear and the norm of time dierivative  $\epsilon_\theta(\vx(t), \sigma(t))$ is unstable, which may lead to the stiffness of the ODE function and the instability of the ODE solver.

Instead, we 


\subsection{Solving semilinear ODEs}

Exponential integrator is initially proposed to solve semilinear problems of the form 
\begin{equation}\label{eq:semi-ode}
    \frac{ \diff \vu(t)} {\diff t} + \mA \vu(t) = \vg(\vu(t), t), \quad \vu(t_0) = \vu_0,
\end{equation}
where $\vu(t) \in \R^n, \mA \in \R^{n\times n}$.

% involve using an initial value and optional temporal midpoints evaluation to estimate the solution at a single time step, while multistep methods involve using multiple previous values to estimate the solution at the next time step. 

\paragraph{Single Step}
The numerical scheme of general single-step methods follows:

\paragraph{Multistep method}
% Another method to approximate unknown non-linear functions 
Multistep method considers another approach to constructing polynomials for approximating unknown non-linear functions. 
Specifically, 

% Derivation for converge condition


% \begin{align}
%     \vu(t_n + c_i h) &= e^{-c_i h \mA} \vu(t_n) + h \sum_{j=1}^{i-1} a_{ij}(-h \mA) \vf(t_n + c_j h) + \Delta _{ni}  \\
%     \vu(t_{n+1}) &= e^{-h \mA} \vu(t_n) + h \sum_{i=1}^s b_i(-h \mA) \vf(t_n + c_i h) + \delta_{n+1} \\
%     \Delta_{ni} &= \sum_{j=1}^{q_i} h^j \psi_{j,i}(-h \mA) \vf^{(j-1)}(t_n) + \Delta_{ni}^{(q_i)} \\
%     \psi_{j,i}(-h\mA) &= \phi_j(-c_i h \mA) c_i^j - \sum_{k=1}^{i-1} a_{ik}(-h\mA) \frac{c_k^{j-1}}{(j-1)!} \\
%     e_n &= \vu_n - \vu(t_n) \\
%     e_{n+1} &= e^{-h_n \mA} e_n - \delta_{n+1} \\
%     \delta_{n+1} &= \sum_{j=1}^p h_n^j \psi_j(-h_n \mA) \vf^{(j-1)}(t_n) + \delta_{n+1}^{(p)} \\
%     \Delta_{ni}^{(q_i)} &= \int_0^{c_i h} e^{-(c_i h -\tau) \mA} 
%     \int_0^{\tau} \frac{(\tau - \sigma)^{q_i - 1}}{(q_i - 1)!} \vf^{(q_i)}(t_n + \sigma) \diff \sigma \diff \tau - h \sum_{k=1}^{i-1} a_{ik}(-h\mA) \int_{0}^{c_k h} \frac{(c_k h - \sigma)^{q_i - 1}}{(q_i - 1)!} \vf^{(q_i)}(t_n + \sigma) \diff \sigma
% \end{align}

\qsh{$\sigma$ vs $\lambda$ linearity}


\subsection{Error recursion~(draft)}

\qsh{sync new and old nations}

\paragraph{Exact solution}

With exact solution $\vx(\lambda)$, we first define $\vf(\lambda) = \mD(\vx(\lambda), \lambda)$ and expand $\vf$ into a Taylor series with remainder in integral form,

\begin{equation}~\label{eq:f-taylor}
    \vf(\lambda_n + \tau) = 
        \sum_{j=1}^q \frac{\tau^{j-1}}{(j-1)!} \vf^{(j-1)}(\lambda_n) + 
        \int_0^{\tau} \frac{(\tau - \nu)^{q-1}}{(q-1)!} \vf^{(q)}(\lambda_n + \nu) \diff \nu
\end{equation}
With~\cref{eq:f-taylor}, we can rewrite exact ODE solution as 
\begin{align}~\label{eq:exact-solution-taylor}
    \vx(\lambda_n + c_i h) &= e^{-c_i h \mA} \vx(\lambda_n) + \sum_{j=1}^{q_i} (c_i h)^j \phi_j(-c_i h \mA) \vf^{(j-1)}(\lambda_n) 
     \\
     &+ \int_0^{c_i h} e^{-(c_i h - \tau) \mA} \int_0^{\tau} \frac{(\tau - \nu)^{q_i-1}}{(q_i-1)!} \vf^{(q_i)}(\lambda_n + \nu) \diff \nu \diff \tau \nonumber,
\end{align}
where function $\phi_j$ is defined as
\begin{equation}\label{eq:def-phi}
    \phi_{j}(-hA) = \frac{1}{h^j} \int_{0}^h \exp^{-(h-\tau)A} \frac{\tau^{j-1}}{(j -1)!} d \tau, \quad j \geq 1
\end{equation}
\begin{equation}\label{eq:phi-recur}
    \phi_{k+1}(z) = \frac{\phi_k(z) - 1 / k!}{z}, \quad \phi_k(0) = \frac{1}{k!}, \quad k \geq 0.
\end{equation}

\paragraph{Exaction solution via numerical scheme}

\begin{subequations}
    \begin{align}
        \vx(\lambda_n + c_i h) &= e^{-c_i h \mA} \vx(\lambda_n) + h \sum_{j=1}^{i-1} a_{ij}(-h \mA) \vf(\lambda_n + c_j h) + \Delta _{ni} \label{eq:single-step-intermediate} \\
        \vx(\lambda_{n+1}) &= e^{-h \mA} \vx(\lambda_n) + h \sum_{i=1}^s b_i(-h \mA) \vf(\lambda_n + c_i h) + \delta_{n+1} \label{eq:single-step-final}
    \end{align}
\end{subequations}
where $\Delta _{ni}$ and $\delta_{n+1}$ are the error terms for intermediate states and final state respectively.

\paragraph{Order conditions based on $\Delta _{ni}$}
Plug in~\cref{eq:f-taylor} into~\cref{eq:single-step-intermediate}, we can obtain
\begin{align}~\label{eq:exact-solution-taylor-single-step-intermediate}
    \vx(\lambda_n + c_i h ) &= e^{-c_i h \mA} \vx(\lambda_n) +
     h \sum_{k=1}^{i-1} a_{ik}(-h \mA) 
     \sum_{j=1}^{q_i} \frac{(c_k h)^{j-1}}{(j-1)!}\vf^{(j-1)}(\lambda_n) 
     \\
     & +
     h \sum_{k=1}^{i-1} a_{ik}(-h \mA) 
     \int_0^{c_k h} \frac{(c_k h - \nu)^{q_i-1}}{(q_i-1)!} \vf^{(q_i)}(\lambda_n + \nu) \diff \nu \diff \tau
     + \Delta _{ni} \nonumber
\end{align}


By comparing~\cref{eq:exact-solution-taylor} and~\cref{eq:exact-solution-taylor-single-step-intermediate}, we can obtain the error term $\Delta _{ni}$ as
\begin{align}
    \Delta_{ni} &= \sum_{j=1}^{q_i} h^j \psi_{j,i}(-h \mA) \vf^{(j-1)}(\lambda_n) + \Delta_{ni}^{(q_i)} \\
    \psi_{j,i}(-h\mA) &= \phi_j(-c_i h \mA) c_i^j - \sum_{k=1}^{i-1} a_{ik}(-h\mA) \frac{c_k^{j-1}}{(j-1)!},
\end{align}
where $\Delta_{ni}^{(q_i)}$ denote higher order terms which resulted from the truncation of the Taylor series.

\paragraph{Order conditions based on $\delta_{n+1}$}
Apply similar techqnique to~\cref{eq:single-step-final}, we can obtain
\begin{align}
    \delta_{n+1} &= \sum_{j=1}^{q} h^j \psi_{j}(-h \mA) \vf^{(j-1)}(\lambda_n) + \delta_{n+1}^{(q)} \\
    \psi_j(-h \mA) &= \phi_j(-h \mA) - \sum_{k=1}^s b_k(-h \mA) \frac{c_k^{j-1}}{(j-1)!},
\end{align}
where $\delta_{n+1}^{(q)}$ denote higher order terms which resulted from the truncation of the Taylor series.


\paragraph{Error recursion}

\begin{align}
    e_n &= \vx_n - \vx(\lambda_n) \\
    E_{ni} &= \vx_{ni} - \vx(\lambda_n + c_i h) \\
    e_{n+1} &= e^{-h \mA} e_n + h \sum_{i=1}^s b_i(-h \mA) (\mD(\vx_{ni}, \lambda_n + c_i h) - \vf(\lambda_n + c_i h)) - \delta_{n+1} \\
    E_{ni} &= e^{-c_i h \mA} e_n + h \sum_{j=1}^{i-1} a_{ij}(-h \mA) 
    (\mD(\vx_{nj}, \lambda_n + c_j h) - \vf(\lambda_n + c_j h)) - \Delta_{ni}
\end{align}


\paragraph{Concrete algorithm}

% \begin{center}
% \begin{tabular}{ c c c c}
% Method & 
%  DEIS~\cite{zhang2022fast} & cell2 & cell3 \\ 
%  cell4 & cell5 & cell6 \\  
%  cell7 & cell8 & cell9    
% \end{tabular}
% \end{center}


% \begin{align}
%     \psi_3(-h \mA) &= 0 \\
%     \sum_{i=1}^s b_i(-h \mA) \psi_{2,i}(-h \mA) &= 0
% \end{align}

% The solution follows

%     and expand $\vf$ into a Taylor series with remainder in integral form,

% \begin{equation}~\label{eq:f-taylor}
%         \vf(\lambda_n + \tau) = 
%             \sum_{j=1}^q \frac{\tau^{j-1}}{(j-1)!} \vf^{(j-1)}(\lambda_n) + 
%             \int_0^{\tau} \frac{(\tau - \nu)^{q-1}}{(q-1)!} \vf^{(q)}(\lambda_n + \nu) \diff \nu
% \end{equation}
% With~\cref{eq:f-taylor}, we can rewrite exact ODE solution as 
% \begin{align}~\label{eq:exact-solution-taylor}
%     \vx(\lambda_n + c_i h) &= e^{-c_i h} \vx(\lambda_n) + \sum_{j=1}^{q} (c_i h)^j \phi_j(-c_i h) \vf^{(j-1)}(\lambda_n) 
%         \\
%         &+ \int_0^{c_i h} e^{-(c_i h - \tau)} \int_0^{\tau} \frac{(\tau - \nu)^{q-1}}{(q-1)!} \vf^{(q)}(\lambda_n + \nu) \diff \nu \diff \tau \nonumber,
% \end{align}
% where function $\phi_j$ is defined as
% \begin{equation}\label{eq:def-phi}
%     \phi_{j}(-h) = \frac{1}{h^j} \int_{0}^h \exp{-(h-\tau)} \frac{\tau^{j-1}}{(j -1)!} d \tau, \quad j \geq 1
% \end{equation}
% On the other hand, 
% where $\Delta _{ni}$ and $\delta_{n+1}$ are the error terms for intermediate states and final state respectively.

% \paragraph{Order conditions based on $\Delta _{ni}$}
% Plug in~\cref{eq:f-taylor} into~\cref{eq:single-step-intermediate}, we can obtain
% \begin{align}~\label{eq:exact-solution-taylor-single-step-intermediate}
%     \vx(\lambda_n + c_i h ) &= e^{-c_i h \mA} \vx(\lambda_n) +
%      h \sum_{k=1}^{i-1} a_{ik}(-h \mA) 
%      \sum_{j=1}^{q} \frac{(c_k h)^{j-1}}{(j-1)!}\vf^{(j-1)}(\lambda_n) 
%      \\
%      & +
%      h \sum_{k=1}^{i-1} a_{ik}(-h \mA) 
%      \int_0^{c_k h} \frac{(c_k h - \nu)^{q-1}}{(q-1)!} \vf^{(q)}(\lambda_n + \nu) \diff \nu \diff \tau
%      + \Delta _{ni} \nonumber
% \end{align}


% By comparing~\cref{eq:exact-solution-taylor} and~\cref{eq:exact-solution-taylor-single-step-intermediate}, we can obtain the error term $\Delta _{ni}$ as
% \begin{align}
%     \Delta_{ni} &= \sum_{j=1}^{q} h^j \psi_{j,i}(-h \mA) \vf^{(j-1)}(\lambda_n) + \Delta_{ni}^{(q)} \\
%     \psi_{j,i}(-h\mA) &= \phi_j(-c_i h \mA) c_i^j - \sum_{k=1}^{i-1} a_{ik}(-h\mA) \frac{c_k^{j-1}}{(j-1)!},
% \end{align}
% where $\Delta_{ni}^{(q)}$ denote higher order terms which resulted from the truncation of the Taylor series.

% \paragraph{Order conditions based on $\delta_{n+1}$}
% Apply similar techqnique to~\cref{eq:single-step-final}, we can obtain
% \begin{align}
%     \delta_{n+1} &= \sum_{j=1}^{q} h^j \psi_{j}(-h \mA) \vf^{(j-1)}(\lambda_n) + \delta_{n+1}^{(q)} \\
%     \psi_j(-h \mA) &= \phi_j(-h \mA) - \sum_{k=1}^s b_k(-h \mA) \frac{c_k^{j-1}}{(j-1)!},
% \end{align}
% where $\delta_{n+1}^{(q)}$ denote higher order terms which resulted from the truncation of the Taylor series.


\subsection{Single-step sampler}



\input{figure/algo/single_sampler}
\input{figure/algo/single_second}
\input{figure/algo/single_third}

\subsection{Multi-step sampler}


\begin{algorithm}[t]
\footnotesize
\captionof{algorithm}[single-step]{\atphantom\ \our SingleStep Order $q$}
\begin{spacing}{1.1}
\begin{algorithmic}[1]
  \AProcedure{SingleSecondSampler}{$D_\theta, ~t_{i \in \{0, \dots, N\}}, c_{2}$}
    \AState{{\bf sample} $\vx_0 \sim \mathcal{N} \big( \mathbf{0}, ~t^2_0 \mathbf{I} \big)$}
        \AComment{Generate initial sample at $t_0$}
    \AFor{$i \in \{0, \dots, N-1\}$}
    %     \AComment{Solve Eq.~\ref{eq:odescale} over $N$ time steps}
        \AState{$\lambda_{i+1}, \lambda_i \gets \lambda(t_{i+1}),  \lambda( t_i)$}
        \AState{$h_i \gets \lambda_{i+1} - \lambda_i$}
            \AComment{Step length}
        % \AState{$a_{21}, b_1, b_2 \gets c_2 \phi_1(-c_2 h), \phi_1(-h) - \phi_2(-h) / c_2, \phi_2(-h) / c_2$}
        \AState{$a_{21}, b_1, b_2 \gets$ \cref{eq:deispp-single-2} with $c_2$}
            \AComment{Runge Kutta coeffients}
      \AState{$\vd_i \gets D_\theta(\vx_i; t_i) -\vx_i $}
            \AComment{Evaluate $\diff\vx / \diff \lambda$ at $(\vx,\,\lambda_i)$}
      \AState{$\vx_{i+1} \gets \vx_i + h(b_1 \vd + b_2 \vd')$}
    \EndFor
    \AState{\textbf{return} $\vx_N$}
        \AComment{Return noise-free sample at $t_N$}
  \EndProcedure
\end{algorithmic}
\end{spacing}
\label{alg:deispp-multi}
\end{algorithm}

\subsection{Butcher tableaus}



\begin{equation}\label{eq:abbr-phi}
    \phi_{i,j} = \phi_{i,j}(-h A) = \phi_i(-c_j hA), \quad 2\geq j \geq s
\end{equation}

% \begin{equation}\label{eq:dpmpp-single-3}
%     \begin{array}{c|ccc}
%          0 \\
%          c_2 & c_2 \phi_{1,2} \\
%          c_3 & 
%          \hline
%          0 & (1 - \frac{1}{2 c_2}) \phi_1 & \frac{1}{2 c_2} \phi_1
%     \end{array}
% \end{equation}


==> sections/body_first_qsh.tex <==
Approximating the data score with a trained denoiser as expressed in~\cref{eq:x0-pred}, the probability flow ODE in \cref{eq:score-sde} (\yc{with $\beta_t = 0$}) simplifies to the following equation:
\begin{equation}~\label{eq:simple-ode}
    \diff \vx = \frac{\vx - \mD_\theta(\vx, \sigma(t))}{\sigma(t)} \dot{\sigma}(t) \diff t. 
\end{equation}
To solve \cref{eq:simple-ode}, ~\citet{karras2022elucidating} interpret the term $\frac{\vx - D_\theta(\vx, \sigma(t))}{\sigma_t} \dot{\sigma}(t)$ as a black box function and choose $\sigma(t) = t$, and then apply a standard second-order Heun ODE solver.
Similarly, \citet{zhang2022fast} consider noise prediction model $\epsilon_\theta(\vx, \sigma(t)) := \frac{\vx - D_\theta(\vx, \sigma(t))}{\sigma_t}$ and leverage existing high order solvers for ODE based on noise prediction model
\begin{equation}~\label{eq:eps-ode}
    \diff \vx = \epsilon_\theta(\vx, \sigma) \diff \sigma.
\end{equation}
They contend that exact solution trajectories $\vx(\sigma)$~\footnote{We utilize $\vx(t)$, $\vx(\sigma)$, and $\vx(\lambda)$ interchangeably when unambiguous, and likewise for $\mD_\theta(\vx, \sigma)$ and $\mD_\theta(\vx, \lambda)$, $\epsilon_\theta(\vx, \sigma)$ and $\epsilon_\theta(\vx, \lambda)$.} in above parameterizations exhibit low curvature and are nearly linear. \yc{why do we have a transition here?
Nevertheless}, in practice, the robustness and stability of the out-of-shelf high-order solvers are critical, necessitating the non-stiffness of the ODE function.
This entails a gradual progression of ODE function evaluations, particularly $\epsilon_\theta(\vx(\sigma), \sigma)$, along the solution trajectory $\vx(\sigma)$~\cite{butcher2016numerical}.
\qsh{do we need a theorem for regular ODE cases to highlight the importance of high order derivative?} \yc{an illustrative example would be helpful}
However, as substantiated by the norm of function derivatives in \cref{fig:function-derivative}, the evolution of $\vf_\eps(\sigma) := \epsilon_\theta(\vx(\sigma), \sigma)$ manifests considerable nonlinearity,  accompanied by an escalating trend as $\sigma \rightarrow 0$. \js{the figure is hard to understand without context?}

\input{figure/viz/function_derivative}

Inspired by ~\citet{kingma2021variational},  we explore an alternative probability flow ODE parameterization by introducing $\lambda_\mD(t) :=- \log \sigma(t)$ based on denoising model $\mD_\theta$.
With $\diff \lambda_\mD(t) = \frac{-\dot{\sigma}(t)}{\sigma(t)} \diff t$, \cref{eq:simple-ode} can be reformulated as follows:
\begin{equation}\label{eq:semi_ode}
    \frac{\diff \vx}{\diff \lambda_\mD} = - \vx + D_\theta(\vx, \lambda_\mD) \quad D_\theta(\vx, \lambda_\mD) := D_\theta(\vx, e^{-\lambda_\mD}).
\end{equation}
A notable advantage of this time rescaling is that the derivative nonlinear function $\vf_\mD (\lambda_\mD) := -\vx + \mD_\theta(\vx, \lambda_D)$ exhibits enhanced smoothness as shown in~\cref{fig:function-derivative}.
Indeed, the smoothness of the nonlinearity function along the solution trajectory, either $\epsilon(\vx(\sigma), \sigma)$ or $\mD(\vx(\sigma), \sigma)$, serves as a crucial determinant of the numerical solver's defects and the sampling quality, as we will demonstrate~later.

Analogously, we can restructure~\cref{eq:eps-ode} by employing a change-of-variables approach with $\vy(t) := \frac{\vx(t)}{\sigma(t)}, \lambda_\eps (t) := \log \sigma(t)$ for the noise prediction model $\epsilon_\theta$:
\begin{equation}\label{eq:semi_ode_eps}
    \frac{\diff \vy}{\diff \lambda_\eps} = - \vy + \eps_\theta(\vy, \lambda_\eps)
    \quad \eps_\theta(\vy, \lambda_\eps) := \eps_\theta(e^{\lambda_\eps} \vy, e^\lambda_\eps).
\end{equation}
We observe that ~\cref{eq:semi_ode,eq:semi_ode_eps} possess highly similar ODE structures, suggesting that ODEs with either epsilon prediction or data prediction models can be addressed within a \textit{unified} framework. 
In fact, ODEs exhibiting the semilinear structure present in \cref{eq:semi_ode,eq:semi_ode_eps}, which comprise a basic linear term and a nonlinear term, are recognized as canonical \textit{semilinear parabolic problems} in the numerical analysis literature\cite{hochbruck2005exponential}.

\yc{we can keep them here, but the texts need to be modified} \qsh{Move to related work? 
    Indeed, \citet{zhang2022fast,lu2022dpm,lu2022dpmp} have also investigated diffusion probability flow ODEs with a comparable semilinear structure, drawing on concepts from exponential integrators to tailor the sampling algorithm for diffusion models. However, in contrast to their work, we demonstrate that with either data prediction or noise prediction models, we can reparameterize ODEs into \textit{canonical} semilinear parabolic problems without time-varying coefficients, enabling the leverage of order analysis from numerical analysis literature to develop enhanced sampling algorithms. As we will reveal later, existing high-order solvers~\cite{lu2022dpm,lu2022dpmp} overlook essential order conditions, resulting in compromised sampling quality and instability in practice.
}

\js{above is replaced in bodyjiaming.tex}
